Canonical Variates in Wasserstein Metric Space

We introduce supervised canonical-variate analysis for distribution-valued observations, where each subject is represented by a probability distribution rather than a single feature vector. We propose the Optimal Transport And Fisher-ratio (OTAF) objective to learn a low-dimensional projection of the ambient feature space by maximizing a Fisher ratio of between-class to within-class variation based on Wasserstein distances. We consider both empirical measures with the 2-Wasserstein distance and fitted Gaussian mixture models (GMMs) with the Minimized Aggregated Wasserstein (MAW) distance. Using the envelope theorem, we derive the objective's gradient and develop a safeguarded gradient-ascent method with a conditional first-order convergence guarantee. We also investigate spectral methods for finding promising starting points by constructing upper bounds on squared Gaussian Wasserstein distances that are quadratic in the projection matrix. We establish bounds relating distribution-estimation error to errors in the Fisher ratio and, under additional assumptions, its maximizing subspace. The analysis distinguishes these estimation effects from optimization error and differences between the Wasserstein and MAW objectives. Controlled simulations and three single-cell applications assess objective values, runtime, initialization sensitivity, and downstream classification performance. The applications demonstrate that OTAF can improve classification in fewer dimensions, with benefits depending on the representation, retained dimension, and downstream classifier.

==> revision_inputs/table_rows.tex <==
1 & 6.8 (0.8) & 7.5 (0.2) & 10.2 (0.8) & 154.9 (32.8) & 497.1 (105.9) & 2172.2 (252.8) \\
2 & 5.4 (0.3) & 6.6 (0.1) & 10.0 (0.2) & 95.8 (3.3) & 391.3 (47.2) & 1610.7 (328.8) \\
3 & 5.6 (0.0) & 7.3 (0.1) & 12.1 (0.5) & 91.4 (4.9) & 328.4 (5.9) & 1300.5 (16.9) \\

